Typing Classes and Mixins with Intersection Types

We study an assignment system of intersection types for a lambda-calculus with records and a record-merge operator, where types are preserved both under subject reduction and expansion. The calculus is expressive enough to naturally represent mixins as functions over recursively defined classes, whose fixed points, the objects, are recursive records. In spite of the double recursion that is involved in their definition, classes and mixins can be meaningfully typed without resorting to neither recursive nor F-bounded polymorphic types. We then adapt mixin construct and composition to Java and C#, relying solely on existing features in such a way that the resulting code remains typable in the respective type systems. We exhibit some example code, and study its typings in the intersection type system via interpretation into the lambda-calculus with records we have proposed.

==> Macros.tex <==
%%%%%%%%%%%%%%%%%%


% Format commands

\newskip \point \point=1pt
\makeatletter

\def\Vec#1{\overrightarrow{#1}}

\def\skp{\hspace*{1\point}}

\newcommand{\mypar}{\medskip \noindent}

% Environments
\newcommand{\TZ}[1]{{#1}}

\newtheorem{definition}{Definition}[section]
\newtheorem{fact}[definition]{Fact}
\newtheorem{ex}[definition]{Example}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{remark}[definition]{Remark}
\newtheorem{conjecture}[definition]{Conjecture}


\newsavebox{\proofbox}
\savebox{\proofbox}{%
  \begin{picture}(7,7)\put(0,0){\framebox(7,7){}}\end{picture}%
}

\newenvironment{proof}
  {\noindent {\it Proof.}}
  {\hspace*{\fill}{\usebox{\proofbox}}\endlist}


% Logic and sets

\newcommand{\defEq}{\stackrel{\Delta}{=}} % = by definition

\newcommand{\Implies}{\Rightarrow} % implication
\newcommand{\Then}{\Rightarrow} % implication
\newcommand{\Iff}{\Leftrightarrow} % logical equivalence
%\newcommand{\And}{\&}

\newcommand{\Set}[1]{\{ #1 \}} % sets
\newcommand{\intersection}{\cap} % intersection
\newcommand{\union}{\cup} % union
\newcommand{\Power}[1]{{\cal P}(#1)}  % powerset


\newcommand{\Nat}{\mathbb{N}} % natural numbers

\newcommand{\dom}{\textrm{\it dom}}

% Domain theory

\newcommand{\dleq}{\sqsubseteq}
\newcommand{\djoin}{\sqcup}
\newcommand{\dJoin}{\bigsqcup}
\newcommand{\dmeet}{\sqcap}
\newcommand{\dMeet}{\bigsqcap}


% Lambda calculus with records

\newcommand{\noop}[0]{\textsf{noop}} % constant for empty operation
\newcommand{\trueVal}[0]{\textsf{true}} % constant true
\newcommand{\falseVal}[0]{\textsf{false}} % constant false

\DeclareMathOperator{\fix}{fix} % fixed point operator

\newcommand{\record}[1]{\ensuremath{{\langle #1 \rangle}}} % record operator
\newcommand{\Pair}[1]{\langle #1 \rangle} % tuple operator (also used for records)

\newcommand{\synteq}{\equiv} % syntactic equality

\newcommand{\NF}{{\cal N}}  % normal forms

\newcommand{\reduces}{\longrightarrow} % one step reduction

\newcommand{\Label}{\mbox{\bf Label}}
\newcommand{\Variable}{\mbox{\bf Var}}

\newcommand{\lambdaR}{\Lambda_R}
\newcommand{\starreduces}{\stackrel{*}{\reduces}}







% Types and type systems

% ground types

\newcommand{\IntType}{\mbox{\sf int}} % integer type (obsolete)
\newcommand{\Int}[0]{\textsf{int}} % integer type
\newcommand{\Bool}[0]{\textsf{bool}} % boolean type
\newcommand{\RealType}{\mbox{\sf real}} % real type
\newcommand{\EvenType}{\mbox{\sf even}} % even integer type
\newcommand{\str}[0]{\textsf{string}} % string type
\newcommand{\unit}[0]{\textsf{unit}} % unit type

% Type constructors

\newcommand{\inter}{\cap} % binary intersection
\newcommand{\bigInter}[2]{\bigcap_{#1} #2} % arbitrary intersection; usage:   \bigInter{indexing}{indexed type expression}


\newcommand{\der}{\vdash} % derivation symbol
\newcommand{\deduces}{\vdash} % derivation symbol (obsolete)

%\newcommand{\Tp}[2]{#1 {\,:\,} #2} %  typing judgement

\newcommand{\arrow}{\rightarrow} % arrow type constructor
\newcommand{\inters}{\wedge} % intersection type constructor

\newcommand{\ArrI}{\arrow\mbox{\it I}}   % arrow introduction 
\newcommand{\ArrE}{\arrow\mbox{\it E}} % arrow elimination
\newcommand{\IntI}{\inter\mbox{\it I}} % intersection introduction
\newcommand{\IntE}{\inter\mbox{\it E}} % intersection elimination
\newcommand{\Axiom}{\textrm{\it Ax}} % axiom rule



% Classes, Mixins etc.

\newcommand{\invoke}[0]{\textit{invoke}}
\newcommand{\myClass}[0]{\textsf{myClass}}
\newcommand{\argClass}[0]{\textsf{argClass}}
\newcommand{\state}[0]{\textit{state}}
\newcommand{\This}[0]{\textsf{this}}  % self parameter; note that \this (lowercase) is in coflict with Taylor's prooftree macros
\newcommand{\self}{\textsf{self}}
\newcommand{\super}{\textsf{super}}

\newcommand{\PointClass}{\textsf{Point}}
\newcommand{\RecPointClass}{\textsf{RecPoint}}
\newcommand{\pointObj}{\textsf{point}}
\newcommand{\PointTwoDMx}{\textsf{Point2D}}
\newcommand{\MovableMx}{\textsf{Movable}}
\newcommand{\movableObj}{\textsf{movable}}
 
\newcommand{\FooMx}{\textsf{Foo}}
\newcommand{\fooObj}{\textsf{foo}}

\newcommand{\Y}{\textbf{Y}}
\newcommand{\send}[2]{#1 \Leftarrow #2}
\newcommand{\get}{\textsf{get}}





% FJ syntax

\newcommand{\kw}[1]{\texttt{#1}}  % keyword

\newcommand{\ClassDeclare}{\texttt{CL}}
%\newcommand{\ConstructDeclare}{}
\newcommand{\ConstructDeclare}{\texttt{K}}
\newcommand{\MethDeclare}{\texttt{M}}
\newcommand{\MethDeclareN}{\texttt{N}}

\newcommand{\Class}{\texttt{C}}  % metavariable of class
\newcommand{\ClassA}{\texttt{A}}
\newcommand{\ClassB}{\texttt{B}}
\newcommand{\ClassC}{\texttt{C}}
\newcommand{\ClassD}{\texttt{D}}
\newcommand{\ClassE}{\texttt{E}}
\newcommand{\ClassF}{\texttt{F}}
\newcommand{\ClassG}{\texttt{G}}
%\newcommand{\ClassBody}[2]{\Set{#1 \ ; \ #2}}
\newcommand{\ClassBody}[3]{\Set{#1; #2; #3}}
\newcommand{\ClassBodyNS}[2]{\Set{#1; \; #2}}
\newcommand{\Object}{\texttt{Object}}

\newcommand{\ClassVar}{\mathtt{X}}
\newcommand{\ClassVarX}{\mathtt{X}}
\newcommand{\ClassVarY}{\mathtt{Y}}

\newcommand{\seq}[1]{\overline{#1}} % a sequence of names, variables
%\newcommand{\emptyseq}{\bullet}
\newcommand{\emptyseq}{\varepsilon}

\newcommand{\field}{\mathtt{f}} % field names
\newcommand{\fieldf}{\mathtt{f}}
\newcommand{\fieldg}{\mathtt{g}}
\newcommand{\fieldh}{\mathtt{h}}

\newcommand{\fieldfunc}[1]{\textit{fields}(#1)}  % field lookup function
\newcommand{\fieldfuncN}[1]{\textit{fldnames}(#1)} 
\newcommand{\mytype}[1]{\textit{mtype}(#1)} % mtype function
\newcommand{\mybody}[1]{\textit{mbody}(#1)} % mbody function

\newcommand{\method}{\mathtt{m}} % method names
\newcommand{\methodn}{\mathtt{n}} 
\newcommand{\var}{\mathtt{x}}  % varaibles
\newcommand{\varx}{\mathtt{x}}  % varaibles
\newcommand{\vary}{\mathtt{y}}  % varaibles
\newcommand{\varz}{\mathtt{z}}  % varaibles
\newcommand{\this}{\texttt{this}} % a special variable, this
\newcommand{\ep}{\mathtt{e}} % expression
\newcommand{\epd}{\mathtt{d}} % expression

\newcommand{\subt}{<:}  % sutype

% Rules (shape)
\newcommand{\fjrule}[1]{{\footnotesize{\ensuremath{[\text{\sc{#1}}]}}}}  % FJ rule

% new macros to be moved as proper


\newcommand{\redSel}{\mbox{\it rsel}}
\newcommand{\redUpd}{\mbox{\it rupd}}
\newcommand{\redMergeThree}{\mbox{\it $\oplus$}}
\newcommand{\recRule}{\mbox{\it rec}}
\newcommand{\selRule}{\mbox{\it sel}}
\newcommand{\updOneRule}{\mbox{\it upd$_1$}}
\newcommand{\updTwoRule}{\mbox{\it upd$_2$}}
\newcommand{\subID}{\mbox{\it s-id}}
\newcommand{\subTrans}{\mbox{\it s-trans}}
\newcommand{\subMap}{\mbox{\it s-map}}
\newcommand{\subRecordOne}{\mbox{\it s-record$_1$}}
\newcommand{\subRecordTwo}{\mbox{\it s-record$_2$}}
\newcommand{\subFunc}{\mbox{\it s-func}}
\newcommand{\tField}{\mbox{\it t-field}}
\newcommand{\tMethod}{\mbox{\it t-method}}
\newcommand{\tBody}{\mbox{\it t-body}}
\newcommand{\tMerge}{\mbox{\it t-merge}}
\newcommand{\tClass}{\mbox{\it t-class}}
\newcommand{\tSub}{\mbox{\it t-sub}}
\newcommand{\tMixin}{\mbox{\it t-mixin}}
\newcommand{\tApp}{\mbox{\it t-app}}
\newcommand{\taRecord}{\mbox{\it ta-rec}}
\newcommand{\taUpd}{\mbox{\it ta-upd}}
\newcommand{\taMerge}{\mbox{\it ta-mrg}}

\newcommand{\Subst}[2]{\{#1 / #2\}}
\newcommand{\ObjToRec}[1]{ \lceil #1 \rceil}
\newcommand{\sigmaupdate}{\leftleftharpoons}
\newcommand{\Sem}[1]{ \langle \! \! \langle #1\rangle \! \! \rangle }


\newcommand{\sigmaAx}{\mbox{\it $\varsigma$-Ax}}
\newcommand{\sigmaOmega}{\mbox{\it $\varsigma$-$\,\omega$}}
\newcommand{\sigmaInter}{\mbox{\it $\varsigma$-$\inter$}}
\newcommand{\sigmaLeq}{\mbox{\it $\varsigma$-$\leq$}}
\newcommand{\sigmaObj}{\mbox{\it $\varsigma$-Obj}}
\newcommand{\sigmaSel}{\mbox{\it $\varsigma$-Sel}}
\newcommand{\sigmaUpdOne}{\mbox{\it $\varsigma$-Upd$_1$}}
\newcommand{\sigmaUpdTwo}{\mbox{\it $\varsigma$-Upd$_2$}}
\newcommand{\converges}[1]{#1 \!\! \downarrow}

\newcommand{\fv}{\mbox{\it fv}}
\newcommand{\New}{\mbox{\sf new}}
\newcommand{\Override}{\;\oplus\;}




%%% eof


==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{Jakob Rehof (Ed.): Intersection Types and Related Systems (ITRS)\\
EPTCS 177, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.177.7}{10.4204/EPTCS.177.7}}
\pdfoutput=1

